ChatPipe: Orchestrating Data Preparation Program by Optimizing Human-ChatGPT Interactions

Orchestrating a high-quality data preparation program is essential for successful machine learning (ML), but it is known to be time and effort consuming. Despite the impressive capabilities of large language models like ChatGPT in generating programs by interacting with users through natural language prompts, there are still limitations. Specifically, a user must provide specific prompts to iteratively guide ChatGPT in improving data preparation programs, which requires a certain level of expertise in programming, the dataset used and the ML task. Moreover, once a program has been generated, it is non-trivial to revisit a previous version or make changes to the program without starting the process over again. In this paper, we present ChatPipe, a novel system designed to facilitate seamless interaction between users and ChatGPT. ChatPipe provides users with effective recommendation on next data preparation operations, and guides ChatGPT to generate program for the operations. Also, ChatPipe enables users to easily roll back to previous versions of the program, which facilitates more efficient experimentation and testing. We have developed a web application for ChatPipe and prepared several real-world ML tasks from Kaggle. These tasks can showcase the capabilities of ChatPipe and enable VLDB attendees to easily experiment with our novel features to rapidly orchestrate a high-quality data preparation program.

==> secs/int_his_man.tex <==
\subsection{Interaction History Management} \label{sec:int_his_man}
This module is used to manage the history of interactions and provides a diff function. For the diff function, given a program $G_1$ and program $G_2$, we first decomposes them into a sequence of lines, namely $g_1=[l^{1}_{1}, l^{1}_{2},…, l^{1}_{n}]$, $g_2=[l^{2}_{1}, l^{2}_{2},…, l^{2}_{m}]$. And we define \textit{change} on the sequence $g$ as $c(g)$, which is to add or delete an element in $g$. We model this problem as a shortest edit script problem ,whose goal is to generate a shortest sequence of changes $C=[c_{1}, c_{2}, …, c_{k}]$, which can transform $g_1$ into $g_2$. 

And inspired by Python diff package\cite{pydiff}, we can use \textit{gestalt pattern matching} algorithm to solve it. Based on it, we prefer to highlight changes in code logic and operations, while ignoring naming differences between different codes. Therefore, we modify the mechanism for comparing two elements (that is, lines of code). In the original algorithm, two elements need to be exactly the same to be considered equal. In our algorithm, we relax this condition. More specifically, the condition that two elements are equal needs to be satisfied:
\be
    \item Except for the variable, the rest of the code line is the same.
    \item If the variables are inconsistent, the data they represent should be the same, that is, generated by two identical pipelines.
\ee

==> secs/materialization.tex <==
\subsection{Execution Acceleration} \label{sec:excute_acceleration}

During the iterative process, various versions of the code for the same ML task is continuously generated. Even if there may be only one operation difference between adjacent versions, users still need to run the entire version from scratch, including those repeated parts, which will cause redundant calculations and lead to high latency. In order to solve this problem and achieve execution acceleration, useful intermediate data will be stored in the cache after each version executed, so that the next version can be directly read from the cache instead of recalculating. 
% We call the way of storing data into the cache materialization, and reading data from the cache as reuse. How to materialize the data set is difficult, because any step of operation may generate intermediate data, the total amount of intermediate data is very large, and the size of the cache is limited. So we need to select valuable data for materialization to maximize benefits. On the other hand, the reuse problem is to make a decision on an whether to reuse an intermediate data or re-calculate it. It is also difficult, and has been proved to be an NP-hard problem\cite{helix}.

Inspired by \cite{helix, CO}, for the materialization problem, we constructed a cost function to estimate whether an intermediate data should be materialized. We used a neural network to model the cost function and optimize it. The features of the cost function include three aspects, namely storage size, computation time and possibility of reuse.

For reuse, we adopt the method of \cite{CO} to solve the problem. 

==> secs/next_ope_rec.tex <==
\subsection{Next Operator Recommendation} \label{sec:next_ope_rec}
 Given a program $G$ and a dataset $D$,  this component outputs a prompt with an operation. It consists of three steps:
 \be
 \item \textbf{Step1 - Program Parsing.} Parse $G$ into pipeline $P$, a DAG with operation as vertex. $P$ can convert $D$ into $D^{\prime}$.
 \item \textbf{Step2 - Operation Selection.} Select an operation $O$ and add it on $P$.
 \item \textbf{Step3 - Prompt Generation.} Convert $O$ into a prompt (text data) $A$, as the output of this component.
\ee

There are two challenges in this component. The first is that it is difficult to convert a program (text data) $G$ into a graph-structured pipeline $P$. It needs to understand the relation in data and operations in $G$. The second is that selecting a quality operation, because there are a variety of operation families (e.g., \term{Imputer} and \term{Scaler}), and within one family, there are many operations (e.g., MinMaxScaler and StandardScaler). Thus, there exist many possible ways of selecting operations to enhance $P$, which are highly dataset-specific and task-specific. 

\stitle{Step1 - Program Parsing.} The program $G$ is parsed in this step into a pipeline $P$. To this end, this step exploits the Abstract Syntax Tree (AST) technique\cite{ast}, like the existing work \cite{haipipe}. Specifically, given a Python program, we parse the program to a pipeline in the following steps.
Fisrt, we split the code into code segments and maintain an ASTNode, which contains the information of the input, operation, output.
Second, we combine individual ASTNodes into a directed acyclic graph based on the data-flow among them i.e.,
connecting two ASTNodes if the output of the former is the input of the latter.

\stitle{Step2 - Operation Selection.} After a pipeline $P$ generated in Step1, this step select an operation $O$ to enhance $P$ to get $P^{\prime}$, which can improve the performance of $P$. First, we introduce operations used in \sys. Next, we introduce how to represent the features. Third, we introduce our optimization algorithm. 
\be
    \item{\textbf{Operations.}} A data prep operation $O$ encapsulates a specific functionality that transforms a dataset $D$ into another dataset $D^{\prime}$, \ie $D^{\prime} = O(D)$. The universe of operations for \sys contains a set of diversified \emph{families} of data prep functionalities, which we called \textit{Logical Operation}, such as \term{Imputer}, \term{Deal Outliers}, \term{Scale}, etc. For each operation in a \textit{Logical Operation $O_{l}$}, we named it \textit{Physical Operation $O_p$}, such as $replace(0, data.median)$ in \term{Deal Outliers}.

    
% Let $\opfamily$ denote the universe of operations for our task $\task$, which contains a set of diversified \emph{families} of data prep functionalities.
% Among them, some rely on well-developed algorithms in known Python libraries, such as Scikit-Learn~\cite{Sklearn}. In this paper, we consider the following families of data prep algorithms implemented in Scikit-Learn (\ie $\term{sklearn}$), likewise in some existing studies~\cite{Deepline,DBLP:conf/kdd/YangFWU20}.

    \item{\textbf{Features Representation.}} This step aims to represent the input data $D$ and $P$ as vectors, to better input them to the optimization algorithm (using deep neural network). 
    \etitle{Dataset embedding $\sttd$} We include statistical information about dataset $D$ in its representation. Each column of $D$ is represented by statistical information. We concatenated them to form $\sttd$. We pad to handle datasets with different column numbers, as neural networks need fixed-size feature vectors.

    % \etitle{Dataset embedding $\sttd$} Same as \cite{haipipe}, we prefer that the dataset representation can contain statistical information of the dataset $D$, because these information can affect the selection of operations to a certain extent. For example, the skewness on columns determines whether we need to do power transformation. Therefore, for each column in the table, we use some statistical information to represent, such as the ratio of missing values, column type, number of unique values, mean etc. Then, we concatenate them to form the dataset feature $\sttd$. Note that since neural networks require fixed-size feature vectors, we use padding to handle datasets with varying numbers of columns.

% \etitle{(1) Dataset embedding $\sttd$} we use statistical information to represent the dataset, which is the same as \cite{haipipe.}

    \etitle{Pipeline embedding $\sttc$} We need to represent both individual vertex and their sequence. For vertex representation, we use a pre-trained program representation model \cite{unixcoder} to represent the partial code of the vertex. For sequence information, we use LSTM\cite{LSTM} to represent the entire pipeline $P$, and finally we use the hidden layer output of the LSTM model as $\sttc$.

    Then we use $s=concat(\sttd, \sttc)$ as the input feature of the optimization algorithm.
% \etitle{(2) Code embedding $\sttc$} We use the public pre-trained code representation model UniXcoder\cite{unixcoder} to represent the code as a vector $\sttc$.
    \item{\textbf{Optimization Algorithm.}} In this step, we introduce how to select an operation $O$ (it can be a \textit{Logical Operation} or a \textit{Physical Operation}.) given $s$. 
    
    \stitle{Policy Function.} The key in this step is to evaluate the ability of an operation that how it can improve current pipeline's performance. 
    In this end, we model two policy function for \textit{Logical Operation} and \textit{Physical Operation} separately, whose input is $s$, and output is a score that measures this ability. The selection process has a hierarchical structure. First, we select a best \term{Logical Operation} through the the \term{Logical Operation} policy function, and next select a best \textit{Physical Operation} through the \textit{Physical Operation} policy function. 
    
    These two policy are optimized by DQN, a Reinforcement Learning framework, with the following elements:
    
    \etitle{State $s$} - the represented vector $s$.
    
    \etitle{Action $a$} - the set of the operations. It is different for \textit{Logical Operation} and \textit{Physical Operation}.
    
    \etitle{Reward $r$} - the executing result of updated code after adding the operation (an action), which is a machine learning evaluation score, such as accuracy. 
    
    \etitle{Termination $t$} - all \textit{Logical Operation} are selected.

    \stitle{Granularity Selection.} After a \textit{Logical Operation} $O_l$ and a \textit{Physical Operation} $O_p$ selected, we need to decide which one is more appropriate in the current state. 
    We can decide by the variance of the policy function's score of operations. When the variance is small, the scores of all \textit{Physical Operations} in $O_l$ are similar, we can recommend $O_l$ and let \plmodel automatically select a \textit{Physical Operation} in $O_l$ (may not be in our \textit{Physical Operation} set); when the variance is large, the $O_p$ is significantly better than other similar \textit{Physical Operations}, and we recommend $O_p$ to \plmodel.

\ee

\stitle{Step3 - Prompt Generation.} After we obtain the specific operation, we built a mapping function to generate corresponding prompts. Note that there are many factors that can cause the execution of programs generated by \plmodel to fail. If this happens, we will use the error message of execution as a prompt for \plmodel in the next iteration.

